Information content of JWST spectra of WASP-39b

WASP-39b was observed using several different JWST instrument modes and the spectra were published in a series of papers by the ERS team. The current study examines the information content of these spectra measured using the different instrument modes, focusing on the complexity of the temperature-pressure profiles and number of chemical species warranted by the data. We examine if H2O, CO, CO2, K, H2S, CH4, and SO2 are detected in each of the instrument modes. Two Bayesian inference methods are used to perform atmospheric retrievals: standard nested sampling and supervised machine learning of the random forest (trained on a model grid). For nested sampling, Bayesian model comparison is used as a guide to identify the set of models with the required complexity to explain the data. Generally, non-isothermal transit chords are needed to fit the transmission spectra of WASP-39b, although the complexity of the Tp-profile required is mode-dependent. The minimal set of chemical species needed to fit a spectrum is mode-dependent as well, and also depends on whether grey or non-grey clouds are assumed. When a non-grey cloud model is used to fit the G395H spectrum, it generates a spectral continuum that compensates for the H2O opacity. The same compensation is absent when fitting the non-grey cloud model to the PRISM spectrum (which has broader wavelength coverage), suggesting that it is spurious. The interplay between the cloud spectral continuum and the H2O opacity determines if SO2 is needed to fit either spectrum. The inferred elemental abundances of carbon and oxygen and the carbon-to-oxygen (C/O) ratios are all mode- and model-dependent, and should be interpreted with caution. Bayesian model comparison does not always offer a clear path forward for favouring specific retrieval models (e.g. grey versus non-grey clouds) and thus for enabling unambiguous interpretations of exoplanet spectra.

==> notes.tex <==
\subsection{(Non?-)confirmation of debated chemical abundances and influence of cloud parameterisation}

In order to compare our results with the detections claimed by ERS works, we note that the accuracy in our outcomes are measured differently. All four ERS studies consider a detection significance parameter $\sigma$, which is converted from the Bayes factor, as in \citet{Trotta2008ConPh..49...71T}. \rev{Analogous to their work, our retrievals using \texttt{Helios-r2} compute Bayes factors based on the difference between their best-fit models with versus without each individual treatment (clouds, temperature-pressure profile, chemistry, and abundance profiles), for both grey and non-grey clouds.}

%However, their works compute Bayes factors based on the difference between their best-fit models with versus without each individual species, one at a time, i.e., considering the model with a species' spectral features, and a second model approximating these features to flat lines.

%In our retrievals using \texttt{Helios-r2}, we take into account the full best-fit model, and our possible detections are based on the posterior distribution of each species favoured by the best-fit model. The abundance of each species is the median values of its posterior inside a 68\% confidence level (1$\sigma$ standard deviation).


\subsubsection{NIRCam}
\rev{Bayesian comparison between models, represented in Fig. \ref{fig:bayes_models}, 
shows our \texttt{Helios-r2} best-fit spectra using NIRCam data for grey and non-grey cloud treatments both favour a \ch{H2O} and \ch{CO2}-only model, with a vertically uniform abundance profile for \ch{H2O}, and a non-uniform, 4-parameter abundance profile for \ch{CO2}, as in Figs. \ref{fig:bayes_models_nonuniform} and \ref{fig:nonuniform}. No additional species are favoured for this instrument. This is expected, as the considered wavelengths cover significant features of \ch{H2O} and \ch{CO2} at 2.7 $\mu$m and 2.8 $\mu$m. Two \ch{H2S} features at about 2.6 $\mu$m and 3.7 $\mu$m are also covered by NIRCam, yet the molecule is not favoured by our analysis. For comparison, \citet{Ahrer2023Natur.614..653A} report the presence of \ch{H2O} in their NIRCam data at a detection significance of 15.9$\sigma$ but no additional detections is mentioned in their results.}

\subsubsection{NIRISS}
\rev{From Fig. \ref{fig:bayes_models}, it is evident that our \texttt{Helios-r2} best-fit spectrum for NIRISS data for grey and non-grey clouds favour the presence of \ch{H2O} and \ch{K}, with 3-parameter non-uniform and uniform abundance profiles, respectively. These are illustrated in Figs. \ref{fig:bayes_models_nonuniform} and \ref{fig:nonuniform}. Our favoured models show no evidence for \ch{CO2}, as the NIRISS wavelength range is at the very end of the 2.8 $\mu$m feature, and does not cover the most significant feature at 4.3 $\mu$m. Additionally, our models do not favour the presence of \ch{CO}, despite the possible feature at 2.4 $\mu$m. Using NIRISS data, \citet{Feinstein2023Natur.614..670F} also claim \ch{H2O} and \ch{K}, at a significance of >30$\sigma$ and 3.6$\sigma$, respectively, with no significant detection of \ch{CO2}. In contrast to our work, they find evidence for \ch{CO} at a significance of 6.8$\sigma$.}

\subsubsection{NIRSpec G395H}
\rev{NIRSpec G395H best-fit models using \texttt{Helios-r2} favour \ch{CO2} and \ch{H2O} only, as seen in Fig. \ref{fig:bayes_models}. Bayesian comparison favours a vertically uniform abundance profile for \ch{H2O} for both grey and non-grey-cloud models, while for \ch{CO2}, non-uniform abundance profiles with 4 and 3 free parameters are preferred for grey and non-grey clouds, respectively. Although the G395H wavelength range covers \ch{H2S}, \ch{SO2}, and \ch{CO} features at 3.7, 4.1, and 4.7 $\mu$m, Fig. \ref{fig:bayes_models} shows these molecules are not favoured by our best-fit models. \citet{Alderson2023Natur.614..664A} also find \ch{CO2} (detection significance of 28.5$\sigma$), \ch{H2O} (21.5$\sigma$), and potentially \ch{SO2} (4.8$\sigma$), but they decline detection of \ch{CO} due to the difficulty in distinguishing from spectral features of \ch{CO2} and \ch{H2O} between 4.4 and 5 $\mu$m.}

\subsubsection{NIRSpec PRISM}
\rev{For NIRSpec PRISM data, covering all probed wavelengths, retrievals using \texttt{Helios-r2} favour both grey and non-grey cloud models with a non-uniform, 2-parameter \ch{H2O} abundance profile. On the other hand, our grey-cloud best-fit model includes uniform profiles for \ch{CO2}, \ch{SO2}, \ch{K}, \ch{H2S}, and \ch{CO}, while our best-fit model for non-grey clouds favour the presence of \ch{CO2}, \ch{K}, and \ch{H2S}, with uniform abundance profiles (see Figs. \ref{fig:bayes_models} and \ref{fig:bayes_models_nonuniform}). \citet{Rustamkulov2023Natur.614..659R} using the NIRSpec PRISM spectrum confirm the presence of \ch{H2O} (detection significance of 33$\sigma$), \ch{CO2} (28$\sigma$), \ch{Na} (19$\sigma$), \ch{CO} (7$\sigma$), and possibly \ch{SO2} (2.7$\sigma$), with no detection of \ch{H2S} and \ch{K}.}
